Probabilistic Directed Distance Fields for Ray-Based Shape Representations

In modern computer vision, the optimal representation of 3D shape continues to be task-dependent. One fundamental operation applied to such representations is differentiable rendering, as it enables inverse graphics approaches in learning frameworks. Standard explicit shape representations (voxels, point clouds, or meshes) are often easily rendered, but can suffer from limited geometric fidelity, among other issues. On the other hand, implicit representations (occupancy, distance, or radiance fields) preserve greater fidelity, but suffer from complex or inefficient rendering processes, limiting scalability. In this work, we devise Directed Distance Fields (DDFs), a novel neural shape representation that builds upon classical distance fields. The fundamental operation in a DDF maps an oriented point (position and direction) to surface visibility and depth. This enables efficient differentiable rendering, obtaining depth with a single forward pass per pixel, as well as differential geometric quantity extraction (e.g., surface normals), with only additional backward passes. Using probabilistic DDFs (PDDFs), we show how to model inherent discontinuities in the underlying field. We then apply DDFs to several applications, including single-shape fitting, generative modelling, and single-image 3D reconstruction, showcasing strong performance with simple architectural components via the versatility of our representation. Finally, since the dimensionality of DDFs permits view-dependent geometric artifacts, we conduct a theoretical investigation of the constraints necessary for view consistency. We find a small set of field properties that are sufficient to guarantee a DDF is consistent, without knowing, for instance, which shape the field is expressing.

==> ddf-theory.tex <==

\newcommand{\bo}{\mathcal{B}}
\newcommand{\boe}{\mathcal{B}_\varepsilon}
\newcommand{\mbo}{$\mathcal{B}$}
\newcommand{\mxi}{$\xi$}

\subsection{Preliminaries}


In this section, our intention is to explore the conditions under which a directed distance field (\acrshort{ddf}), or one of its constituent fields, represents a shape. 
In particular, we show an equivalence between certain local properties of such fields and the existence of a 3D shape to which the field has been perfectly ``fitted''.
We begin by defining the basic setting, including the domain in which our fields operate, the oriented points that characterize our ray-based geometric representation, 
and the precise definition of a shape. 


\begin{mydef}{Domain $\bo$, $\boe$, $\Gamma$, and $\Gamma_\varepsilon$}{pddf:prelim:domain}
We consider fields with a geometrically simple domain, $\bo \subset \real^3$.
In particular, we assume that \mbo \ is convex, compact, and has a smooth boundary, $\partial \bo$,
with outward-facing surface normals.
Finally, 
for $\varepsilon > 0$,
we denote $\boe$ as the $\varepsilon$-domain of $\bo$, defined via 
\begin{equation}
	\boe = \left\{ p \in \bo \,\middle\vert\, 
	\min_{b\in\partial\bo} || p - b || \geq \varepsilon \right\},
\end{equation}
which will be useful for ensuring certain boundary conditions on our fields of interest.

Often, we will be interested in the 5D Cartesian product space, $\Gamma = \bo \times \mathbb{S}^2$.
Similarly, we can define $\Gamma_\varepsilon = \boe \times \mathbb{S}^2$.
\end{mydef}

The role of $\boe$ is to enable us to define a notion of 
``away from the boundary''
	(i.e., $\bo\setminus\boe$ is a thin $\varepsilon$-width shell around the edges of the domain).
Notice that we restrict our attention to a small part of $\real^3$, 
	where our shape of interest will reside,
	but the domain of our fields will be the 5D space $\Gamma$, 
	comprising oriented points or, equivalently, rays.

\begin{mydef}{Oriented Points and Rays}{pddf:prelim:orienrays}
	We generally denote an \textit{oriented point} via
	$\tau = (p,v) \in \Gamma$ (or in $\Gamma_\varepsilon$ when specified).
	Any oriented point induces (or is equivalent to) a 3D \textit{ray}: $r_\tau(t) = p + tv,\, t\geq 0$.
	In a slight abuse of notation, we may refer to the oriented point and ray forms of such 5D elements interchangeably. 
\end{mydef}

Fundamentally, our interest is in representing 3D shapes, 
	which are defined simply as follows.
	
\begin{mydef}{Shapes}{pddf:prelim:shape}
	We define a \textit{shape} to be a compact set $S\subset \bo$.
	Often, we will be interested in shapes 
		$S \subset \boe$,
	for $\varepsilon > 0$.
\end{mydef}

Note that using $\boe$ does not strongly constrain the shape: for example, one can simply use the bounding sphere of the given point set, and then inflate it enough to satisfy the $\varepsilon$ condition.

Next, for the sake of notational simplicity, we define an ``along-ray'' form of any function (or field) that operates on oriented points (i.e., in 5D), by considering its restriction to a given ray.

\begin{mydef}{Along-Ray Functions}{pddf:prelim:alongray}
	We define the ``along-ray'' form of a function
	$ g : \Gamma \rightarrow \mathcal{X} $,
	which maps into a set $\mathcal{X}$, to be:
	\begin{equation}
		f_g(s\mid \tau) := g(p + sv, v) = g(r_\tau(s), v),
	\end{equation}
	where $s \geq 0$, $\tau = (p,v) \in \Gamma$, and
	$r_\tau$ is the ray form of $\tau$.
\end{mydef}

Finally, we introduce notation for the intersections of rays and point sets.
\begin{mydef}{Intersecting Rays and Point Sets}{pddf:prelim:intersections}
	Consider a point set $S\subseteq \bo$ and an oriented point $\tau\in\Gamma$.
	
	\textit{Intersected Points}.
	Let $S_\tau\subseteq S$ denote the set of points in $S$ intersected by $r_\tau$
	(i.e., $q\in S_\tau$ iff $\,\exists\; t\geq 0$ such that $r_\tau(t) = q$).
	For notational convenience, we may write $[S]_\tau$ as well.
	
	\textit{Intersecting Rays}.
	Let $\mathcal{I}_S \subseteq \Gamma$ be the set of rays 
	that intersect at least one member of $S$
	(i.e., $\tau \in \mathcal{I}_{S}$ if $\exists\; q\in S$ such that $r_\tau(s) = q$ for some $s\geq 0$).
	For $q\in\bo$, we denote $ \mathcal{I}_{q} := \mathcal{I}_{\{q\}} $.
\end{mydef}


\subsection{View Consistency for Simple DDFs}

Our first consideration will be a simplified form of \acrshort{ddf}, 
	which does not utilize a visibility field.

\begin{mydef}{NNBC Field}{pddf:simple:nnbc} \index{NNBC field}
An \textit{NNBC field} on $\Gamma$ is a \underline{n}on-\underline{n}egative, \underline{b}ounded scalar field that is piece-wise \underline{c}ontinuously differentiable along rays, 
written $ d : \Gamma \rightarrow \real_{\geq 0} $. 
The latter condition means the along-ray form is piecewise $C^1$ 
(i.e., it satisfies $f_d(s\mid p,v) = d(p + sv,v) \in C^1$).
\end{mydef} 

In general, such fields need not have an obvious connection to any shapes (in the sense of the definition above).
In this section, we treat such fields as \textit{putative} representations for shapes -- the goal is to understand the exact conditions under which such fields are ``equivalent to'' (or ``represent'') some shape.

\begin{mycdef}{Positive Boundary Condition for Simple DDFs (BC$_d$)}{pddf:simple:bcd}
	An NNBC field $d$ satisfies the \textit{Positive Boundary Condition} BC$_d$ iff
	\begin{equation}
	\inf_{v\in\mathbb{S}^2} d(p,v) > 0 \;\forall\; p\in \bo\setminus\boe.		
	\end{equation}	
\end{mycdef}

Recall that $\bo\setminus\boe$ is the ``outer shell'' of the bounding domain. In other words, BC$_d$ demands that $d$ cannot have any zeroes close to $\partial\bo$. 

\begin{mycdef}{Directed Eikonal Condition for Simple DDFs (DE$_d$)}{pddf:simple:ded}
An NNBC field $d$ satisfies the \textit{Directed Eikonal Constraint} DE$_d$ if
$\partial_s f_d(s\mid\tau) = -1$, except at along-ray zeroes of $d$ 
(i.e., at any $(q,v)$ such that  
$\lim_{\epsilon \downarrow 0} \inf_{s\in (0,\epsilon)}
d(q - sv, v) = 0$).
\end{mycdef}

The second constraint is on the derivative of $d$:
	it says that, along any ray, $d$ must decrease linearly, at unit rate, unless $d=0$ (a value at which it may potentially stay).

\begin{mycdef}{Isotropic Opaqueness Condition for Simple DDFs (IO$_d$)}{pddf:simple:iod}
	An NNBC field $d$ satisfies the \textit{Isotropic Opaqueness Constraint} at a point 
	$q\in\bo$ if
	\begin{equation}
		\left(
		\lim_{\epsilon \downarrow 0} 
		\inf_{ \substack{s\in (0,\epsilon)\\ v\in\mathbb{S}^2 } }
		d(q - sv, v) = 0
		\right)
		\,\implies\,
		\left(
		\lim_{\epsilon \downarrow 0} \inf_{s\in (0,\epsilon)}
		d(q - sv, v) = 0
		\,\forall\, v\in\mathbb{S}^2\right).    
		\label{eq:iod}
	\end{equation}
We say $d$ is isotropically opaque, denoted IO$_d$, if it satisfies the Isotropic Opaqueness Constraint everywhere in $\bo$.
\end{mycdef}

Notice that this is stronger than (i.e., it implies) the following constraint,
	which refers only to local properties 
	in the neighbourhood of some oriented point $(q,v)$:
\begin{equation}
	\left(
	\exists\,v\in\mathbb{S}^2 \;\mathrm{s.t.}\; 
	\lim_{\epsilon \downarrow 0} \inf_{s\in (0,\epsilon)}
	d(q - sv, v) = 0
	\right)
	\,\implies\,
	\left(
	\lim_{\epsilon \downarrow 0} \inf_{s\in (0,\epsilon)}
	d(q - sv, v) = 0
	\,\forall\, v\in\mathbb{S}^2
	\right).
\end{equation}

Namely, if the field approaches zero at some position $q$ from \textit{any} direction $v$, then it must approach zero at that point from \textit{all} directions.
Note that, for the left-hand side of Eq.~\ref{eq:iod}, 
a single particular direction $v$ along which $d$ converges to zero need not exist 
(see Appendix \S\ref{pddf:theory:convergenceexample} for an example).
The weaker, second form of IO$_d$ means that convergence to a zero from one direction must be accompanied by a zero from all directions.

Together, these field constraints enable us to define a \textit{simple \acrshort{ddf}}, which we will show is capable of representing shapes with theoretical consistency guarantees.

\begin{mydef}{Simple DDF}{pddf:simple:simpleddf} \index{simple DDF}
	We define a simple DDF to be an NNBC field such 
	that IO$_d$, BC$_d$, and DE$_d$ are satisfied.
\end{mydef}

The remainder of this section will be devoted to showing that
	the three field constraints, which define a simple \acrshort{ddf},
	are sufficient to ensure a form of ``view consistency''.

Before that, however, we define some notational constructs around Simple \acrshort{ddf}s.
First,
	we define a simple function based on $d$,
	which outputs the \textit{position}
	that our depth field takes us to, along a given ray.
\begin{mydef}{Positional Field}{pddf:simple:q}
	Any simple DDF has an associated positional field, or $q$-mapping, defined by:
	$q(p,v) := p + d(p,v) v$.
\end{mydef}

Next, because \acrshort{ddf}s can be discontinuous at zeroes,
	for convenience of notation, 
whenever a simple DDF $d$ approaches zero along a ray, 
we denote this as a zero of the field (regardless of the nature of any discontinuities at such points).

\begin{mydef}{Left-Continuity Convention}{pddf:simple:leftcont}
For any $q\in\boe$, we write:
\begin{equation}
	d(q,v) = 0 
	\,\iff\,
	\lim_{\epsilon \downarrow 0} \inf_{s\in (0,\epsilon)}
	d(q - sv, v) = 0. \label{eq:contconv}
\end{equation}
\end{mydef}

In words, left continuity for $d$ defines a slightly looser notion of a zero along rays (here, we say ``left'' with respect to the direction $v$).
We also apply this convention to $q$, so that if $d(p,v)=0$, we write $q(p,v) = p$.
Finally, we define a special set of points that is associated to any simple \acrshort{ddf}.

\begin{mydef}{Positional Zero Set for Simple DDFs}{pddf:simple:zeroes}
	We denote the set of \textit{positional zeroes} of a Simple DDF as
	\begin{equation}
		Q_d = %
		\left\{ p\in\bo \;\middle\vert\; %
		\lim_{\epsilon \downarrow 0} 
		\inf_{ \substack{s\in (0,\epsilon)\\ v\in\mathbb{S}^2 } }
		d(p - sv, v) = 0 \right\}.
	\end{equation}
\end{mydef}

Note that the condition for being in $Q_d$ is slightly weaker than that of being a directional zero, 
in the sense of Eq.~\ref{eq:contconv}.
I.e., there may be $q \in Q_d$ such that 
	there is no $v$ for which $d(q,v) = 0$.
However, any $q$ that satisfies $d(q,v) = 0$ for some $v$ is necessarily in $Q_d$.

Our first lemma concerns these positional zeroes, 
	namely that it is a closed set bounded in $\boe$.

\begin{restatlem}{Properties of Simple DDF Positional Zeroes}{pddf:simple:closedinboe}
	Let $d$ be a simple \acrshort{ddf}.
	Then $Q_d \subseteq \boe$ and $Q_d$ is a closed set.
\end{restatlem}
\begin{proof}
	See Appendix \S\ref{pddf:theory:propposzeroes}.
\end{proof}

Notice this shows that $Q_d$ is a shape 
	(i.e., compact point set).
We will use these properties later, 
	connecting this point set to the shape 
	represented by the field (as we will later show).
The first step along this line is to define what it means 
	for a simple \acrshort{ddf} to ``exactly'' represent a shape.


\begin{mydef}{Shape-Induced Simple DDFs}{pddf:simple:shapeinduction}
	Let $S$ be a shape such that $S\subseteq\boe$. 
	We define a set of ``induced fields'' associated to $S$, which each act as a form of \textit{representation} for the shape.
	Recall that $S_\tau$ denotes the points in $S$ intersected by $r_\tau$.
	Then $ S $ \textit{induces} a field $ d : \Gamma \rightarrow \real_{{\geq}0} $
	iff \\
	(i) for any $\tau=(p,v)\in\Gamma$ such that $S_\tau \neq \varnothing$,
	$d(\tau) = \min_{q \in S_\tau} ||q - p||$
	and \\
	(ii) $\exists\; \varepsilon_E > 0$ such that
	for any $\tau\in\Gamma$ with $S_\tau = \varnothing$, 
	we have that $d(\tau) > \varepsilon_E $, $q(\tau) \notin \bo $, and $f_d$ is $C^1$ along $r_\tau$ with 
	$ \partial_s f_d(s \mid \tau) = -1 $.
	
\end{mydef}

Intuitively, a point set $S$ induces a field $d$ if (i) the $q$-mapping always takes $p$ to the closest point in $S$ along $v$, unless (ii) no intersection exists, in which case $q$ must predict a point \textit{outside} the valid domain. 
Notice, of course, that a large class of $d$ can therefore satisfy this for a given $S$, differing only in where outside \mbo\  they output.\footnote{
	An alternative form of shape-induction (see Appendix \S\ref{pddf:theory:altfieldind}) avoids defining notions of equivalence by including the boundary $\partial\bo$ with the shape $S$. This enables a simpler form of equality, but the approach above is more analogous to what we will do in the case of the full \acrshort{ddf}.
}
We next show that any induced field is a Simple DDF.

\begin{restatthm}{Shape-Induced Fields Are Simple DDFs}{pddf:simple:sifsasdds}
Consider a field $d$ that is induced by some shape $S$.
Then $d$ is a simple DDF. 
Further, the positional zeroes of $d$ in $\bo$ satisfy $S = Q_d$.
\end{restatthm}
\begin{proof}
	See Appendix \S\ref{pddf:theory:sifasd}.
\end{proof}

Recall that the definition of a shape-induced field need not be unique (as two induced fields may differ on rays that do not intersect $S$) and therefore allows a given $S$ to induce a \textit{set} of $d$ fields, which differ only in terms of their out-of-domain behaviour. 
Hence, we need a measure of ``equivalence'' between Simple DDFs.
A given shape $S$ can then induce an equivalence class of Simple DDFs.
To define this notion of equivalence, we first define the set of empty rays.

\begin{mydef}{Empty Rays}{pddf:simple:emptyrays}
Let $d$ be a Simple DDF.
Then we let
$\mathcal{E}[d] \subseteq \Gamma$ be the set of \textit{empty rays}, defined by 
$ \mathcal{E}[d] = \{ \tau \in \Gamma \mid q(\tau)\notin \bo \} $, where $q$ is the $q$-mapping of $d$.
Notice that an empty ray $\tau \in \mathcal{E}[d]$ must have 
$f_d(s\mid \tau) > 0$ as long as $r_\tau(s) \in \bo$.
(I.e., we cannot have a zero of $d$ on an empty ray). 
\end{mydef}

For a given $d$, 
	the empty rays are those that $d$ maps outside of the domain.
To check equality,
	we can ignore the depth \textit{values} of empty rays,
	as long as \textit{which} rays are empty is the same.

\begin{mydef}{Equivalence of Simple DDFs}{pddf:simple:equiv}
	Consider two Simple DDFs, $d_1$ and $d_2$. 
	Then $d_1$ and $d_2$ are \textit{equivalent} iff
	(i)
	both fields have the same set of empty rays, written $\mathcal{E}$ 
	(i.e., $ \mathcal{E} := \mathcal{E}[d_1] = \mathcal{E}[d_2] $)
	and
	(ii) 
	they agree on non-empty rays
	(i.e., $d_1(\tau) = d_2(\tau)\;\forall\; \tau \in \Gamma \setminus \mathcal{E}$).
\end{mydef}

Later we will see a slightly different form of equivalence 
	between \textit{full} DDFs 
	(i.e., including a visibility field), 
	similar to that of Simple DDFs.
First, however, we formally define what it means for a simple DDF to be a shape representation.

\begin{mydef}{Shape Representations as View-Consistent Simple DDFs}{pddf:simple:shaperep}
    A Simple DDF $d$ is View Consistent (VC)
	iff
	there exists a shape $S$ such that 
	$S$ induces $d$.
	
	We can therefore call any such $d$ a \textit{shape representation} for the point set $S$.
\end{mydef}

Recall that an NNBC field (see Def.~\ref{df:pddf:simple:nnbc})
	maps rays (in 5D) to positive scalars, with very little constraints.
Most such fields will not be view-consistent, 
	in the sense that they will not represent a shape (point set), 
	in a self-consistent manner
	(e.g., violating the basic inequality\footnote{
		Recall that if $q(p_1,v_1)$ is a predicted surface point,
		then $d(p_2,v_2) \leq || p_2 - q(p_1,v_1) ||$, 
		for any ray $r_{(p_2,v_2)}$ that intersects $q(p_1,v_1)$. 
	} 
		from \S\ref{pddf:appendix:viewconsis}).
The definition above formalizes what it means for a field to 
be view-consistent.

The next theorem is the main result of this section.
It shows that the local\footnote{Local in the sense that each constraint can be defined about a single point, particularly IO$_d$ (a point that is zero along one ray must be zero on all of them) and DE$_d$ (the along-ray derivative at any point is $-1$). } field constraints (Constraints \ref{cdf:pddf:simple:bcd}, \ref{cdf:pddf:simple:ded}, and \ref{cdf:pddf:simple:iod}) are sufficient to ensure a Simple DDF represents a shape (i.e., in a view-consistent manner).

	
\begin{restatthm}{Every Simple DDF is a Shape Representation}{pddf:simple:esdiasr}
Any simple DDF $d$ 
is view consistent 
(i.e., there exists a shape $S \subseteq \boe$ such that $d$ is equivalent to any field induced by $S$).
Further, 
$d$ is a shape representation for the set formed by its positional zeroes, $Q_d$
(i.e., $Q_d$ induces $d$).
\end{restatthm}
\begin{proof}
	See Appendix \S\ref{pddf:theory:esdiasr}.
\end{proof}

The two theorems above
(\ref{th:pddf:simple:sifsasdds} and \ref{th:pddf:simple:esdiasr})
show that being a simple DDF 
(i.e., non-negativity, no zeroes close to the boundary, isotropic zeroes, and unit along-ray derivatives) 
is equivalent to view consistency (i.e., to being induced by some shape).
In other words, 
the constraints on the implicit field of being a simple DDF is synonymous with being a shape representation.
Later, these results will be useful when showing that \textit{full} DDFs 
	can be constrained in a similar manner, 
	in order to guarantee view consistency.

\subsection{View Consistency for Visibility Fields}

We next look at the second constituent field in a DDF: the visibility field, which demarcates whether or not a shape is present along a given ray. Similar to the previous section, our interest is in determining sufficient constraints on a given visibility field such that one can be assured it is ``view-consistent'', meaning compatible with some 3D shape. 

As for simple \acrshort{ddf}s, we begin by defining a relatively unconstrained field,
	for which we shall find constraints relating to view consistency.

\begin{mydef}{BOZ Field}{pddf:vis:bozf} \index{BOZ field}
Let $\xi : \Gamma \rightarrow \{ 0, 1 \}$ be a binary-valued field on $\Gamma$. 
We restrict $\xi$ such that its zero set is open; i.e.,
$\forall \; \tau \in \Gamma$, if $\xi(\tau) = 0$, then $\exists\; \varepsilon > 0$ such that $\xi(\widetilde{\tau}) = 0 \;\forall\; \widetilde{\tau} \in B_{\varepsilon}(\tau) \cap \Gamma $, where $B_{\varepsilon}(\tau)$ is the open ball centered at $\tau$ of radius $\varepsilon$.

We call any such \underline{b}inary field, with an \underline{o}pen \underline{z}ero set, a BOZ field.
\end{mydef}

Similar to NNBC fields (Def.~\ref{df:pddf:simple:nnbc}), a BOZ field does not have an obvious connection to 3D shapes or their multiview silhouettes -- one can  imagine BOZ fields that do not represent a consistent 3D point set from all viewpoints.
Our goal is to understand when (or under what conditions) a BOZ field acts as a continuous representation of the silhouettes of some coherent shape
(i.e., when it assigns every ray a binary indication 
as to whether a shape point exists along that ray or not).
It turns out a very similar situation to that of Simple DDFs arises.
Thus, similarly, we begin by defining field constraints,
	which will eventually connect BOZ fields to coherent silhouettes of shapes. 

\begin{mycdef}{Non-Visible Boundary Condition for Visibility Fields (BC$_\xi$)}{pddf:vis:bcxi}
	A BOZ field $\xi$ satisfies the 
	\textit{Non-Visible Boundary Condition},
	denoted BC$_\xi$, if
	$\xi(p,v) = 0 \;\forall\; (p,v)\in 
	\mathcal{O}[\bo\setminus\boe, \boe]$,
	where 
	$\mathcal{O}[V,U] = \{ \tau=(p,v) \in\Gamma \mid p\in V, r_\tau(s) \notin U \;\forall\; s\geq 0 \}$ is the set of ``outward rays'' from a given set.
\end{mycdef}
Recall that $\bo\setminus\boe$ is the ``outer shell'' of the bounding domain and, essentially, $\mathcal{O}[V,U]$ contains oriented points (or, equivalently, rays) that \textit{start} in $V$ and do \textit{not} intersect $U$.
In other words, BC$_\xi$ demands that any rays that (i) start at a point close to the boundary and (ii) do not intersect the inner part of the domain (i.e., $\boe$) must have a value of zero. 
Intuitively, if we imagine $\xi$ to be representing an object in $\boe$, 
this condition prevents the object from being visible on rays 
that start outside of $\boe$ and ``look away'' from $\boe$.

\begin{mycdef}{Directed Eikonal Constraint for Visibility Fields (DE$_\xi$)}{pddf:vis:dexi}
A BOZ field $\xi$ satisfies the \textit{Directed Eikonal Constraint} DE$_\xi$ 
if
$\xi$ is always non-increasing along a ray
(i.e., $ f_\xi(s_1|\tau) \leq f_\xi(s_2|\tau) \;\forall \tau \in \Gamma, s_1 > s_2$ ).
\end{mycdef}
Intuitively, along a ray, this constraint means that the visibility can only ever go from ``seeing'' to ``not seeing'' an object 
(i.e., along a ray, one should not suddenly see a new point in the shape become visible).

\begin{mycdef}{Isotropic Opaqueness for Visibility Fields (IO$_\xi$)}{pddf:vis:ioxi}
A BOZ field $d$ satisfies the \textit{Isotropic Opaqueness Constraint} at a point $q\in\bo$ if
the following implication holds:
\begin{align}
	&\left(
	\exists\; v\;\mathrm{s.t.}\; 
	\lim_{\epsilon\downarrow 0} \sup_{s\in(0,\epsilon)}
	\xi(q - sv,v) = 1
	\;\land\;
	\lim_{\epsilon\downarrow 0} \inf_{s\in(0,\epsilon)}
	\xi(q + sv,v) = 0
	\right) \nonumber \\
	\;&\;\;\implies\;
	\big(
	\xi(\tau) = 1
	\;\forall\;\tau \in \mathcal{I}_q 
	\big), 
\end{align}
where $\mathcal{I}_q $ is the set of rays in $\bo$
(i.e., $r_\tau$, for oriented points $\tau\in\bo$)
that intersect $q$.
An \textit{isotropically opaque field} (IO$_\xi$) satisfies the Isotropic Opaqueness Constraint everywhere.	
\end{mycdef}

In words, if there is \textit{any} direction 
along which the field flips from one to zero,
then the point at which that occurs must be ``isotropically opaque''
(i.e., from any direction, any ray that hits that point must produce a visibility value of one).
Intuitively, IO$_\xi$ says that 
	such ``one-to-zero`` discontinuities in $\xi$ are special. 
As we shall see, they act similar to surface points 
(or zeroes of $d$, in the case of simple DDFs).
In particular, for any point $q\in\bo$, 
if even a single direction $v$ exists such that 
a one-to-zero discontinuity occurs along $v$ at $q$, then any ray that contains $q$ must also be visible.    

As for simple \acrshort{ddf}s, with these three constraints,
	we can now define an appropriately limited set of fields, 
	called visibility fields,
	which we will show is intimately tied to shapes.

\begin{mydef}{Visibility Field}{pddf:vis:visibilityfields}
We define a Visibility Field to be a BOZ field such that
	IO$_\xi$, BC$_\xi$, and DE$_\xi$ are satisfied.	
\end{mydef}

Analogously to simple \acrshort{ddf}s with left continuity (Def.~\ref{df:pddf:simple:leftcont}), 
we utilize a notational convention for visibility, 
which slightly broadens when an oriented point is considered visible.

\begin{mydef}{Upper-Continuity Convention for Visibility Fields}{pddf:vis:uppercont}
Whenever a visibility field $\xi$ approaches one, 
we denote the field value as one, regardless of the nature of any discontinuities at such points.
In particular, for any $q\in\bo$, 
we write:
\begin{equation}
	\xi(q,v) = 1 
	\,\iff\,
	\lim_{\epsilon \downarrow 0} 
	\sup_{ \substack{ || \delta || < \epsilon \\ q + \delta \in \bo } } 
	\xi(q + \delta, v) = 1.
	\label{eq:contconv:vis}
\end{equation}
\end{mydef}
In other words, we assume ``upper continuity'' for $\xi$, along all directions.
Notice that this is consistent with the requirement on BOZ fields that the zero set $\xi^{-1}(0)$ is open.
Further, its complement, $\xi^{-1}(1) \subseteq \Gamma = \bo\times\mathbb{S}^2$, is closed (using the fact that $\bo$ is compact).

\newcommand{\closure}{\mathscr{C}}

\begin{mydef}{Positional Discontinuities of the Visibility Field}{pddf:vis:posdiscont}
Consider a visibility field $\xi$. 
Then we define its positional discontinuity set as follows:
\begin{equation}
Q_\xi :=
\closure %
\left(
	\left\{
		q \in \bo
		\;\middle\vert\;
		\exists\; v\;\mathrm{s.t.}\; 
		\lim_{\epsilon\downarrow 0} \sup_{s\in(0,\epsilon)}
		\xi(q - sv,v) = 1
		\;\land\;
		\lim_{\epsilon\downarrow 0} \inf_{s\in(0,\epsilon)}
		\xi(q + sv,v) = 0
	\right\}
\right),\nonumber
\end{equation}  
where $\closure$ is the closure operator on sets.
\end{mydef}
Intuitively, given a visibility field $\xi$, the set $Q_\xi$
simply contains all of the one-to-zero discontinuities in $\xi$.
More specifically, for any point $q\in\bo$, 
if there exists some direction $v$ such that the field $\xi$
flips from one to zero 
(i.e., from ``seeing something'' to ``seeing nothing'') 
at $q$,
then $q\in Q_\xi$.

\begin{restatlem}{Properties of Positional Discontinuities of Visibility Fields}{pddf:vis:posdiscont}
A visibility field $\xi$ satisfies 
(i) $Q_\xi \subseteq \boe$,
(ii) $Q_\xi$ is a shape, and 
(iii) there cannot be discontinuities in $\xi$ from zero-to-one along a ray.
\end{restatlem}
\begin{proof}
	See Appendix \S\ref{pddf:theory:posdiscont}.
\end{proof}

Given these properties, the discontinuities $Q_\xi$
	are a good candidate for a potential shape that
	$\xi$ is implicitly representing.
First, like for simple \acrshort{ddf}s, 
	we need to define what it means for a shape 
	to \textit{induce} a field 
	(i.e., ``exactly'' represent it).

\begin{mydef}{Shape-Induced Binary Fields}{pddf:vis:sibfs}
Let $S\subseteq\boe$ be a shape. 
Recall that $\mathcal{I}_{S} \subseteq\Gamma$ is the set of rays that intersect $S$.
Then we say a BOZ field $\xi$ %
	is \textit{induced} by $S$ if the following holds:
\begin{equation}
	\xi(\tau) = 1 \;\iff\; \tau \in \mathcal{I}_{S}.
\end{equation}
Further, given a fixed shape $S$, its associated induced field $\xi$ is unique.
\end{mydef}

Notice that the induction relation is an ``iff'', 
	meaning $\xi(\tau) = 0$ implies that \textit{no} $q\in S$
	can be present along the ray $r_\tau$.
In addition, importantly, while the $S$-induced field $\xi$ is unique,
	the inducing shape for a given $\xi$ is \textit{not} necessarily unique.
For instance, imagine a sphere with another shape (say, another sphere) inside it -- such a shape will induce the same visibility field as using the outermost sphere alone for the inducement. 
Given this definition,
	our first result in this section shows that any shape-induced field 
		satisfies the constraints of a visibility field.
\begin{restatthm}{Shape-Induced Binary Fields Are Visibility Fields}{pddf:vis:sibfavf}
Let $S\subseteq \boe$ be a shape, with an induced field $\xi$.
Then $\xi$ is a visibility field 
(i.e., IO$_\xi$, BC$_\xi$, and DE$_\xi$ hold).
Further, the positional discontinuities of $\xi$ satisfy $Q_\xi \subseteq S$.
\end{restatthm}
\begin{proof}
	See Appendix \S\ref{pddf:theory:sibfavf}.
\end{proof}

\newcommand{\xirepname}{{indicator}}
\newcommand{\Xirepname}{{Indicator}}

So far we have shown that any shape can be used to generate or induce 
	a visibility field (in the sense of Def.~\ref{df:pddf:vis:visibilityfields}).
We can use this to define a notion of shape representation for visibility fields.

\begin{mydef}{Shape {\Xirepname}s as View-Consistent Visibility Fields}{pddf:vis:shaperep}
A visibility field $\xi$ is View Consistent (VC) iff there exists a shape $S$ 
such that $S$ induces $\xi$.
We can therefore call  
any such $\xi$ a \textit{shape} \textit{{\xirepname}} for the point set $S$.
\end{mydef} \index{shape indicator}
Note we call it a shape indicator instead of a representation because we cannot (necessarily) reconstruct $S$ from $\xi$ (i.e., it would be an incomplete representation). Instead, we call it an {\xirepname} because it ``indicates'' whether or not the shape (or some shape) exists along the given ray
(i.e., acts as an indicator function for each ray). 
We next show that the local constraints of a visibility field
	are sufficient for it to be a representation of some shape.
\begin{restatthm}{Every Visibility Field is a Shape \Xirepname}{pddf:vis:evfias}
Let $\xi$ be a visibility field.
Then there exists a point set $S$ such that $\xi$ is induced by $S$.
Further, we can take the positional discontinuities as an inducer; 
	i.e., $S := Q_\xi$ induces $\xi$.
\end{restatthm}
\begin{proof}
	See Appendix \S\ref{pddf:theory:evfias}.
\end{proof}

So far, we have shown a close duality between visibility fields
and shape indicators (i.e., between binary fields with specific local constraints on the field, namely IO$_\xi$, DE$_\xi$, and BC$_\xi$, and binary fields constructed from a given point set).
However, it is clear that many inducing point sets can induce the same field.
Unlike the case with simple DDFs, 
	this is not merely a question of behaviour outside the domain
	(e.g., recall the example of a sphere within a sphere inducing the same field as the outer sphere alone).
We can therefore ask for a ``minimal example'' over an equivalence class of inducing point sets
(i.e., given many shapes $S$ that all induce the same $\xi$, which is the simplest?).

This leads us to the following corollary, which shows that
	the simplest (i.e., smallest) shape (i.e., closed point set)
	that induces a given
	visibility field is the set of positional discontinuities.

\begin{restatcor}{Minimal Characterization of Visibility Fields}{pddf:vis:minimalcharvis}
Consider the set of shapes 
$ \mathfrak{S}[\xi] = \{ S \mid S\subseteq\bo \;\text{induces}\; \xi \}$ 
that all induce the same field $\xi$.
I.e., $\mathfrak{S}[\xi]$ is an equivalence class of inducing shapes.
Then, $Q_\xi \in \mathfrak{S}[\xi]$ is the smallest closed point set among all such inducers.
\end{restatcor}
\begin{proof}
	See Appendix \S\ref{pddf:theory:minimalcharvis}.
\end{proof}

This shows that $Q_\xi$ is special among shapes that induce $\xi$,
	in that it forms a subset of any other shape that also induces $\xi$.
Next, we provide some additional intuition concerning $Q_\xi$, 
	which is derived from the visibility field itself.
Instead, given any shape $S$, we can describe which subset of points
	actually forms $Q_\xi \subseteq S$, 
	without referring to any $\xi$ directly.

\begin{mydef}{Directly Lit Points}{pddf:vis:dlp} \index{Directly Lit Points}
	Consider a shape $S$ contained in $\boe$.
	Imagine a set of uniform lights placed at each $p\in\partial\bo$
	(or, equivalently, imagine each such $p$ casting rays in all possible directions.
	We denote the set of points in $S$ that are ``directly lit'' by such lights
	(or intersected \textit{first} by such cast rays) as
	$\mathfrak{D}_\ell(S)$.
	Mathematically, the directly lit points (DLPs) can be written
	\begin{equation}
		\mathfrak{D}_\ell(S) = 
		\closure
		\left(
		\left\{
		q \in S \;\middle\vert \;
		\exists\;\tau = (p,v)\in\Gamma_\partial
		\,\;\mathrm{s.t.}\;
		q = \arg\min_{ \widetilde{q} \in S_\tau } || p - \widetilde{q} ||
		\right\}\right),
	\end{equation}
	where $\Gamma_\partial = \partial\bo\times \mathbb{S}^2$ and 
	$S_\tau$ is the set of points in $S$ that are intersected by the ray $r_\tau$.
\end{mydef}

Intuitively, any point in $S$ that can be hit by a light ray from the boundary, 
directly and without occlusion,
is a DLP.
One could, equivalently, call $q\in \mathfrak{D}_\ell(S)$ 
an \textit{observable} point from the boundary.
Similar to $Q_\xi$, 
we include a closure operator, 
to ensure that $ \mathfrak{D}_\ell(S) $ 
contains its limit points and boundary.
Without this, the directly lit set is not necessarily closed.

We next show that directly lit points are an alternative characterization of the positional discontinuities.
Intuitively, it relates the local field property of a one-to-zero discontinuity
to the ``observable'' behaviour of the shape from the boundary $\partial \bo$.
In other words, DLPs are defined via the point set $S$, 
\textit{not} its induced field $\xi$. 
However, we next show that $\mathfrak{D}_\ell(S)$ is a special subset of $S$,
in that it forms a minimal inducer for the equivalence class $\mathfrak{S}[\xi]$,
and it is therefore equal to $Q_\xi$.

\begin{restatcor}{Directly Lit Points Minimally Characterize Visibility Fields}{pddf:vis:dlpsareqxi}
Given any shape $S$ in the equivalence class $\mathfrak{S}[\xi]$ of inducers for the field $\xi$,
the set of DLPs $\mathfrak{D}_\ell(S)$ is a \textit{minimal} inducer of $\xi$
and furthermore $\mathfrak{D}_\ell(S) = Q_\xi$.
\end{restatcor}
\begin{proof}
	See Appendix \S\ref{pddf:theory:dlpsareqxi}.
\end{proof}

In words, to get the minimal inducing point set from a shape $S$, one need not construct the induced field and then find its discontinuities. 
Instead, one can compute the DLPs directly from $S$, by ``looking inwards'' from the boundary and finding the observable (i.e., directly lit) points.

\textbf{Summary.}
We have shown that 
(i) we can devise a notion of ``inducement'', under which any 3D shape gives rise to an associated visibility field, $\xi$, which acts as its binary indicator function along rays;
(ii) the local constraints that define a visibility field $\xi$ 
(i.e., IO$_\xi$, DE$_\xi$, BC$_\xi$) are sufficient to guarantee that 
\textit{some} point set must exist that induces $\xi$
(meaning, every visibility field is the indicator of some shape);
(iii) the positional discontinuities $Q_\xi$ play a special role, as the \textit{minimal} closed subset of $S$ that can induce a given field $\xi$
(in some sense, $Q_\xi$ represents the best reconstruction of the initial shape that one can obtain from $\xi$); and
(iv) an alternative but equivalent characterization of the minimal closed inducing subset of $S$ can be given by the set of directly lit points (DLPs).

\subsubsection{Shape-from-Silhouette, Visual Hulls, and Visibility Fields}

The connection to DLPs (or boundary-observable points) allows us to interpret $\xi$ more intuitively as the continuous field of silhouette images.
In this setting, each pixel is associated to a ray that starts, say, from a camera outside the domain,
and assigns a binary pixel value that decides whether or not the given shape is intersected by that ray.
As already noted, given $\xi$, one can compute $Q_\xi$, which recovers as much information about the shape (or, rather, the equivalence class of shapes) that could have induced it as is possible.
This is therefore closely related to 
	prior work on shape-from-silhouette and visual hulls, 
	which has seen significant theoretical investigation in prior works. 

In particular, estimating 3D shape from visibility images alone (i.e., silhouettes) has been studied in computer vision for decades \cite{baumgart1974geometric} 
(see also \cite{cheung2005shape}), 
complemented by research into how humans overcome 
the inherent ambiguity of the problem
(e.g., \cite{marr1980visual,willatsl1992seeing}).
Given that an infinite set of shapes can give rise to an identical silhouette,
additional constraints are needed for shape inference, 
either in the form of purely geometric considerations \cite{richards1987inferring}, 
priors \cite{li2018single}, or simply more viewpoints. 
In general,
the basic idea is to use back-projection from the silhouettes into 3D space,
with each such constraint forming a 3D \textit{visual cone},
in which the shape must lie.
The volumetric intersection of such cones generates the \textit{visual hull} of the object, a point set that contains the shape of interest with increasing precision as the number of views increases.
Significant theoretical work has characterized the geometry of visual hulls,
particularly in the shape-from-silhouette context
(e.g., \cite{laurentini1994visual,laurentini1995far,laurentini1997many,laurentini1999computing,petitjean1998computational,trager2016consistency,kutulakos1997shape}).
Numerous techniques have been applied to visual hull computation
(e.g., \cite{lazebnik2001computing,lazebnik2007projective,landabaso2008shape,yi2007efficiently}),
as well as applications thereof
(e.g.,  %
\cite{matusik2000image,furukawa2009carved,franco2006visual}).
Generalizations of the shape-from-silhouette problem consider 
errors in the camera poses, inconsistencies or noise in the silhouettes themselves,
or issues related to non-convexity of shapes
(e.g., \cite{bottino2003introducing,haro2012shape,cheung2000real,landabaso2008shape,zheng19923d,zheng1994acquiring}).
Space carving \cite{kutulakos2000theory} 
generalizes shape-from-silhouette geometric constraints 
to utilize a notion of photo-consistency, 
producing a ``photo-hull'' that is more constrained than the visual hull;
this relates more closely to recent AbS approaches to multiview 3D scene reconstruction,
such as NeRFs (see, e.g., \S\ref{relwork:implicitshape}).

In contrast, our work focuses on potentially under-constrained 5D visibility fields,
which can be rendered into silhouettes from any continuously varying viewpoint, 
and the conditions under which such fields properly correspond to some underlying shape
(i.e., when $\xi$ is a shape representation, guaranteeing view consistency).
The most common shape-from-silhouette situation involves so-called \textit{external} visual hulls, which involve only viewpoints (i.e., cameras) outside the convex hull of the shape \cite{laurentini1994visual}.
In the context of this thesis, a visibility field $\xi$ considers the presence of a shape along any possible ray.
This enables $\xi$ 
to represent aspects of shape that are missed by external visual hulls,
such as concavities,
and is thus more similar to \textit{internal} visual hulls 
(e.g., see \cite{petitjean1998computational,laurentini1994visual}),
which assigns the ``viewing region'' to be anywhere outside the shape 
(not just its convex hull).

Nevertheless, questions still arise regarding visibility fields and their representational capacity.
One aspect of shapes ``missed'' by visibility fields is \textit{internal structure}:
shape points that are completely surrounded by other shape points cannot be preserved by the field.
In other words, given a shape $S$ with internal structure, 
any $S$-induced field will not be able to recover such structure.\footnote{
	This is why there is an equivalence class of shapes that induce a given visibility field 
	(i.e., $\mathfrak{S}[\xi]$).}
One can see this by noting that 
the directly lit points of $\xi$ 
(equivalently, the set of one-to-zero discontinuities)
will not include such internal structure.
These points, however, fully encode the field (as they induce it).
Combining a visibility field with a distance field, as we will do in the next section, enables a complete shape representation (i.e., including internal structure).

\subsection{View Consistency for Directed Distance Fields}

In this section, we investigate the \textit{combination} of a visibility field and a slightly modified form of simple DDF,
which define the full DDF discussed in the other sections of this chapter.
Similar to the prior two sections, 
we define view consistency through a notion of ``shape representation''; 
i.e., whether or not some shape (point set) exists that induces the DDF.
In this case, the visibility field will be used to control where 
(in $\Gamma$) 
the distance field needs to be strongly constrained. 
This is different from the simple DDF case,     
in that it alleviates constraints on $d$.
Given a simple DDF, 
one can imagine constructing a visibility field based on the presence or absence of a zero of the $d$-field along the ray (i.e., whether $q$ maps a ray outside of $\bo$).
However, this section considers the opposite: rather than deriving $\xi$ from $d$, we specify $\xi$ first, and use it to derive where and how $d$ must be constrained (reducing the demands on $d$).
As a result of this, 
we need additional conditions to ensure that the visibility field and depth field are compatible with one each other.

\newcommand{\visrays}{\mathcal{R}_V}
\newcommand{\nonvisrays}{\mathcal{R}_N}



\begin{mydef}{Visible and Non-Visible Ray Sets}{pddf:full:vnvrs}
	Let $\xi$ be a visibility field.
	We define the sets of visible and non-visible rays, respectively, as
	\begin{align}
		\visrays[\xi]    &= \{ \tau \in \Gamma \mid \xi(\tau) = 1 \} \\
		\nonvisrays[\xi] &= \{ \tau \in \Gamma \mid \xi(\tau) = 0 \}, 
	\end{align}
	written via upper-continuity (Def.~\ref{df:pddf:vis:uppercont}).
	Further, $\visrays[\xi]$ is closed, 
		while $\nonvisrays[\xi]$ is open.
\end{mydef}

The closed or open nature of these sets
is due to the BOZ field definition, which requires %
$\xi^{-1}(0)$ to be open,
and so its complement 
$\xi^{-1}(1)\subseteq \Gamma = \bo\times \mathbb{S}^2$ is closed,
since $\Gamma$ is compact.

\begin{mydef}{$\xi$-Coherent Simple DDFs}{pddf:full:xicoherent}	
Given a visibility field $\xi$,
an NNBC field $d$ is a $\xi$-coherent simple DDF
iff it satisfies %
\begin{enumerate}
	\item [(IO$_{d,\xi}$)]
	\textit{Isotropic opaqueness on visible rays.}
	\begin{equation}
		\forall\;
		(q,v)\in\visrays[\xi]: \;
		\lim_{\epsilon \downarrow 0} 
		\inf_{ \substack{s\in (0,\epsilon)\\ v\in\mathbb{S}^2 } }
		d(q - sv, v) = 0
		\,\implies\,
		d(q,v) = 0. %
	\end{equation}
	\item [(BC$_{d,\xi}$)]
	\textit{Positive boundary condition on visible rays.}
	\begin{equation}
		\big(
		(p,v)\in \visrays[\xi] \,\land\, 
		p\in \bo\setminus\boe
		\big)
		\,\implies\,
		d(p,v) > 0 .
	\end{equation}
	\item [(DE$_{d,\xi}$)]
	\textit{Directed Eikonal constraint on visible rays.}
	
	For any $\tau\in\visrays[\xi]$ such that
	$d(\tau) > 0$, we have $ \partial_s f_d(s\mid\tau)|_{s=0} = -1 $.
\end{enumerate}	
\end{mydef}

In words, a $\xi$-coherent depth field $d$ satisfies the
isotropic opaqueness, boundary, and directed Eikonal constraints
whenever $\xi = 1$ (i.e., it is a simple DDF on $\visrays[\xi]$).
Outside of the visible rays $\visrays[\xi]$, $d$ is essentially unconstrained.

\newcommand{\lvz}{Q_{d,\xi}}

\begin{mydef}{Locally Visible Depth Zeroes}{pddf:full:lvdz}	
Let $\xi$ be a visibility field and $d$ be $\xi$-coherent.
Then the \textit{locally visible zeroes} are given by
\begin{equation}
	\lvz = 
	\closure
	\left(\left\{
	\widetilde{q} \in Q_d  
	\; \middle\vert \;
	\exists\, v \in \mathbb{S}^2 
	\;\mathrm{s.t.}\;
	\xi(\widetilde{q}, v) = 1
	\right\}\right),
\end{equation}
where 
$\closure$ is closure and
we use upper-continuity %
for $\xi$ (Def.~\ref{df:pddf:vis:uppercont}). %
\end{mydef}
This set includes any zero of $d$ 
(i.e., $q\in Q_d$; see Def.~\ref{df:pddf:simple:zeroes})
that is ``locally visible'' along some direction 
(meaning, 
$\lim_{\epsilon\downarrow 0}\sup_{||\delta|| < \epsilon} \xi(q + \delta,v) = 1$).
The locally visible zeroes ($\lvz$) will play an analogous role
to the zeroes $Q_d$ for simple DDFs
and the discontinuities $Q_\xi$ for visibility fields.

\begin{mydef}{Directed Distance Field (DDF)}{pddf:full:fullddf}	
A BOZ field $\xi$ and an NNBC field $d$ form a 
\textit{Directed Distance Field} $(\xi,d)$ iff:
\begin{enumerate}
	\item 
	$\xi$ is a visibility field.
	\item 
	$d$ is a $\xi$-coherent simple DDF.
	\item 
	Locally visible depth zeroes are isotropically opaque with respect to $\xi$:\\
	$q \in \lvz$ $\implies$ 
	$ \tau \in\visrays[\xi] \;\forall\; \tau\in\mathcal{I}_q $,
	where 
	$\mathcal{I}_q\subset \Gamma$ is the set of rays that intersect $q$.
	\item 
	Every visible ray must hit a locally visible depth zero:\\
	$ \tau \in\visrays[\xi] \implies \bo_\tau \cap \lvz \ne \varnothing$,
	where $\bo_\tau$ is the set of points in $\bo$ 
	intersected by $r_\tau$.
\end{enumerate}
\end{mydef}

The definition of a DDF can be intuited as combining a visibility field with a simple DDF that is constrained only along visible rays, 
along with two additional restrictions that force the two to be consistent.
The consistency constraints hinge on special zeroes of $d$ 
that are ``locally visible'' 
(i.e., at least one ray exists, 
along which $q\in Q_d$ is visible at an infinitesimal distance).
Such zeroes are (i) always visible and (ii) every visible ray must intersect at least one.
The next lemma clarifies the relation between the fundamental point-sets associated with these various fields: the zeroes of $d$, the visibility discontinuities, and the locally visible depth zeroes.

\begin{restatlem}{Fundamental Point Sets}{pddf:full:fundps}
Let $(\xi,d)$ be a DDF. Then $Q_{\xi} \subseteq \lvz \subseteq Q_d$.
\end{restatlem}
\begin{proof}
	See Appendix \S\ref{pddf:theory:fundps}.
\end{proof}

Note that locally visible zeroes (i.e., points in $\lvz$) require all intersecting rays to be visible rays, but they do \textit{not} require such points to be one-to-zero visibility discontinuities (i.e., $Q_\xi$). 
However, such discontinuities \textit{do} have to be 
zeroes of the depth field
	(i.e., in $Q_d$).

Next, we connect the locally visible depth zeroes to a closely related set of points, the directly visible zeroes, where the relation is more non-local.
Later, this relation will be useful in determining the relationship between shape-induced field tuples (soon to be defined, in Def.~\ref{df:pddf:full:inducedfieldpair}) and DDFs.

\newcommand{\dvdz}{\mathcal{D}_{d,\xi}}

\begin{mydef}{Directly Visible Depth Zeroes}{pddf:full:dvdz}	
Let $(\xi,d)$ form a DDF.
Then the set of \textit{directly visible depth zeroes} is given by
\begin{equation}
	\dvdz = 
	\closure
	\left(\big\{
	\widetilde{q} \in\bo  
	\; \big\vert \;
	\exists\,  (p,v) \in \visrays[\xi] 
	\;\mathrm{s.t.}\;
	q(p,v) = \widetilde{q}
	\big\}\right),
\end{equation}
where $q(p,v)$ is the $q$-mapping of $d$.
	
\end{mydef}
In words, $\dvdz\subseteq \bo$ records positions where
at least one ray $\tau$ exists such that
(i) $\xi(\tau) = 1$ and
(ii) $\widetilde{q}$ is the \textit{first} zero (i.e., member of $Q_d$) along $r_\tau$.
Thus, equivalently, using the properties of $\xi$-coherence,
we may write
\begin{equation}
	\dvdz = 
	\mathrm{Closure}\left(\big\{
	\widetilde{q} \in\bo  
	\; \big\vert \;
	\exists\, \tau \in \visrays[\xi] 
	\;\mathrm{s.t.}\;
	\widetilde{q}
	=
	p + \widetilde{s}(\tau\mid Q_d) v
	\big\}\right),
\end{equation}
where $\widetilde{s}(\tau\mid S) = \min_{q \in S_\tau} || p - q ||$, $\tau = (p,v)$,
and $S_\tau$ is the set of points in $S\subseteq\bo$ that are intersected by $r_\tau$.
This latter form helps illuminate the connection to shape induction 
	(e.g., recall Def.~\ref{df:pddf:simple:shapeinduction} 
		for simple \acrshort{ddf}s).
First, however, we show that not only are
	the locally and directly visible depth zeroes 
	equivalent, but 
	that the outputs of $d$ and $q$ (the positional field of $d$)
	are effectively controlled by
	them.

\begin{restatlem}{DDFs Map to Locally Visible Depth Zeroes}{pddf:full:dmdvdz}
Let $(\xi,d)$ be a DDF. Then $\lvz = \dvdz$.
Further:
\begin{equation}
	\forall\;\tau = (p,v) \in\visrays[\xi]:\;
	d(\tau) = \min_{ \widetilde{q} \in [\dvdz]_\tau } || \widetilde{q} - p ||
	\,\;\text{and}\;\, q(\tau) \in \lvz,
\end{equation}
where $[\dvdz]_\tau$ is the set of points in $\dvdz$ that intersect $r_\tau$ and $q$ is the $q$-mapping of $d$.
\end{restatlem}
\begin{proof}
	See Appendix \S\ref{pddf:theory:dmdvdz}.
\end{proof}
This lemma will be used later, to link \acrshort{ddf}s to shape representations.
Following the previous two sections, on simple DDFs and visibility fields, 
we next define an approach to ``field induction'': 
given a shape $S$, how can we construct a DDF, 
consisting of a ``field pair'' $(\xi,d)$,
that appropriately represents $S$?
We then show that inducing a field in this manner, versus having a DDF with constraints on local field behaviour 
(i.e., Def.~\ref{df:pddf:full:fullddf})
are equivalent.

\begin{mydef}{Induced Field Pair}{pddf:full:inducedfieldpair}	
Consider a shape $S \subseteq \boe$.
By Def.~\ref{df:pddf:vis:sibfs}, $S$ induces a unique visibility field, $\xi$.
We also define an induced distance field $d$ to be any NNBC field that satisfies 
\begin{equation}
	d(\tau) = \min_{q\in S_\tau} ||q - p||
	\;\forall\; 
	\tau\in\visrays[\xi],
\end{equation}
where $S_\tau$ is the set of points in $S$ that are intersected by $r_\tau$.

Then, given a shape $S$, 
we define any such pair $(\xi,d)$, 
to be an \textit{induced field pair}.
\end{mydef}

Notice that this construct for $d$ is similar to inducement of simple DDFs; 
	the main difference is that $d(\tau)$ is unconstrained when $\xi(\tau) = 0$ 
	(i.e., $d$ no longer needs to predict distances outside the domain).
Further, the induced visibility $\xi(\tau)$ is one iff $\tau$ intersects $S$. 
Hence, for a visible ray $\tau\in\visrays[\xi]$, 
	   $d$ is constrained to always predict the distance to 
	   the closest $q\in S_\tau$.

Thus, similar to Theorems \ref{th:pddf:simple:sifsasdds} and \ref{th:pddf:vis:sibfavf}, 
	when a shape $S$ induces a field pair $F$, 
	we want to show that $F$ follows the field requirements of \acrshort{ddf}s 
	(Def.~\ref{df:pddf:full:fullddf}).

\begin{restatthm}{Induced Field Pairs are Directed Distance Fields}{pddf:full:ifpaddfs}
Let $S$ be a shape and $F=(\xi, d)$ be an $S$-induced field pair.
Then $F$ is a Directed Distance Field, which satisfies $\lvz = S$.	
\end{restatthm}
\begin{proof}
	See Appendix \S\ref{pddf:theory:ifpaddfs}.
\end{proof}

Now that we know that any field pair generated from a shape is a \acrshort{ddf},
	we next want to work towards showing the converse, 
	that any \acrshort{ddf} is a shape representation of some shape.
First, similar to simple \acrshort{ddf}s, the presence of the visibility field
	means we need to define a notion of equivalence between fields
	(where values on non-visible rays can be ignored).

\begin{mydef}{Equivalence of Directed Distance Fields}{pddf:full:equivddf}	
Consider two DDFs, $F_1 = (\xi_1,d_1)$ and $F_2 = (\xi_2,d_2)$.
Then $F_1$ and $F_2$ are equivalent iff
(i) $\xi_1(\tau) = \xi_2(\tau)\;\forall\; \tau\in\Gamma$
and 
(ii) $d_1(\tau) = d_2(\tau) \;\forall\; \tau\in\visrays[\xi_1]$.
\end{mydef}

This definition of field equality enables us to establish when a \acrshort{ddf} is a shape representation.

\begin{mydef}{View Consistent Directed Distance Fields as Shape Representations}{pddf:full:shapereps}	
A DDF $F$ is view consistent (VC) iff it is equivalent to a DDF that has been induced by a shape $S$.
I.e., $F$ is VC iff there exists a shape $S$ such that 
$F$ is an $S$-induced field pair.
In such a case, 
we say that \textit{$F$ is a shape representation for $S$}.
\end{mydef}

Finally, 
analogously to Theorems~\ref{th:pddf:simple:esdiasr} and \ref{th:pddf:vis:evfias},
we can assert that the field constraints of Def.~\ref{df:pddf:full:fullddf}
	are sufficient to guarantee that a \acrshort{ddf} represents some shape.

\begin{restatthm}{Every Directed Distance Field is a Shape Representation}{pddf:full:eddfiasr}
Let $F=(\xi,d)$ be a DDF. %
Then $F$ must be view consistent 
(i.e., there exists a shape $S$ such that $F$ is an $S$-induced field pair).
Further, $\lvz$ is a shape that induces $F$.
\end{restatthm}
\begin{proof}
	See Appendix \S\ref{pddf:theory:eddfiasr}.
\end{proof}

This last theorem finally links \textit{full} DDFs to shape representations, by combining view-consistent visibility fields with depth fields that are constrained (in the same manner as simple DDFs) along visible rays (i.e., in $\visrays[\xi]$) and \textit{un}constrained along non-visible rays (i.e., in $\nonvisrays[\xi]$).
In other words, full DDFs are simple DDFs, 
but with looser requirements on $d$ when $\xi = 0$ (controlled instead by a visibility field, $\xi$).
The concept of shape representation can therefore be equivalently derived in two ways: (i) by starting from a point set and inducing a field pair from it, or (ii) by starting from a visibility field and a distance field that are ``compatible'' with one another, and satisfying the basic requirements on the fields (BC, IO, and DE).

The latter case, in particular, is important, as it suggests that
one need only ensure certain local constraints,
	in order to obtain a view consistent 5D field.
Specifically, for the boundary conditions (BC), 
one should demand that, 
near the boundary of the domain,
$d$ does not predict surface points (i.e., zeroes) and
the visibility field returns zero whenever it ``looks outward'' from the domain (i.e., the shape cannot be visible outside the domain).
For the directed Eikonal (DE) constraints, one requires $\partial_s f_d = -1$ and $f_\xi$ non-increasing, along visible and all rays, respectively.
Isotropic opaqueness (IO)
asks that (visible) zeroes of $d$ are zero from all directions and, similarly, that one-to-zero ``flips'' in $\xi$ are visible from all directions.
Finally,
two demands are placed to ensure consistency between the visibility and depth fields, relying on the set of locally visible zeroes 
(i.e., depth zeroes that are visible at infinitesimally close points along some ray):
(a) any ray that intersects such a zero must be visible, 
and 
(b) any visible ray must hit such a zero.
Together, the previous theorems ensure that a field satisfying these conditions must be a shape representation (and vice-versa).


This is reminiscent of solving the Eikonal equation to obtain a distance field,
which is loosely followed by some modern distance-based isosurface \acrshort{isf} training methods (see \S\ref{pddf:appendix:proofs:prop1}).
Notice, for instance, that BC and IO act like boundary conditions, 
	while DE forms the constraint that needs to be solved across space.
We expect that improvements in techniques 
for fitting higher-dimensional \acrshort{inr}s with differential constraints
(in this case, equivalent to solving a 5D partial differential equation)
will make neural implementation of (P)DDFs more viable.


In summary, these theorems give requirements for generic learned fields 
(i.e., implemented as neural networks $(\xi_\theta,d_\theta)$ with weights $\theta$)
that ensure view-consistency if satisfied.
By careful design of the field architectures and losses, 
to ensure fitting to the data and satisfaction of these conditions, 
we should converge to the desired shape,
given enough network capacity and sufficient supervision.














